Hidden in Plain Sight: Evaluating Abstract Shape Recognition in Vision-Language Models

Despite the importance of shape perception in human vision, early neural image classifiers relied less on shape information for object recognition than other (often spurious) features. While recent research suggests that current large Vision-Language Models (VLMs) exhibit more reliance on shape, we find them to still be seriously limited in this regard. To quantify such limitations, we introduce IllusionBench, a dataset that challenges current cutting-edge VLMs to decipher shape information when the shape is represented by an arrangement of visual elements in a scene. Our extensive evaluations reveal that, while these shapes are easily detectable by human annotators, current VLMs struggle to recognize them, indicating important avenues for future work in developing more robust visual perception systems. The full dataset and codebase are available at: \url{https://arshiahemmat.github.io/illusionbench/}

==> chapters/checklist.tex <==
%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Statements are reiterated throughout \Cref{sec:zs_exp}, \Cref{sec:icl_exp} and \Cref{sec:mdg_exp}}
  \item Did you describe the limitations of your work?
    % \answerYes{See \Cref{sec:limitations}}
    \answerYes{In associated experimental sections (e.g., \Cref{sec:icl_exp})} and in \Cref{app:dataset_limitations}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See \Cref{sec:impact}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes, we are not violating any ethics review guideline. We discuss potential negative societal impacts.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See supplementary materials and \url{https://huggingface.co/datasets/arshiahemmat/IllusionBench} (also linked in abstract)}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \cref{app:fullzeroshot},\cref{app:icl_full}, \cref{app_mdg_full}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Re-running large-scale experiments multiple times would have introduced a prohibitive cost, given the scale and scope of our experiments.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{In \cref{app:misc} }
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{In \cref{app:extra_data_details}}
  \item Did you mention the license of the assets?
    \answerYes{In \cref{app:extra_data_details}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{In the Abstract (as a footnote with URL)}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{In \cref{app:extra_data_details}}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
  \answerNo{None of our data contains PII or offensive content (see \Cref{sec:data_details})}

\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{In \cref{app:extra_data_details}}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{In \cref{app:extra_data_details}}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


\newpage
\mbox{~}

==> chapters/limits.tex <==


% \paragraph{In-Context Learning} Current multi-modal in-context learners struggle to adapt to complex tasks beyond standard benchmarks such as VQA. As multi-modal ICL is still developing, future models may exhibit improved ICL capabilities, enabling better detection of abstract shapes and disentanglement of shape and scene prediction. 
% We leave these investigations for future work to investigate.

% \paragraph{Optical Character Recognition (OCR)} 
% {\org
% We also generated a comparable dataset with text represented in images instead of non-character symbols. 
% While annotators were able to consistently recognize text {\red at X\% accuracy (whatever it is)}, we observed highly inconsistent behaviors among the VLMs we tested: all open-source VLMs achieved zero or near-zero accuracy, and the only models that achieved nontrivial performance were black-box API-only models trained on unknown data. {\red can we lump them in as also being "near-zero" or is their performance sufficiently nontrivial (e.g., let's say higher than 5\%)?} 
% Due to the difficulties associated with evaluating on this dataset -- including, e.g., how to account for multiple possible tokenizations of character strings, whether to assign ``partial credit'' for some (but not all) of the correct characters, whether and how to compare models that have been trained on OCR tasks against those that have not, etc. -- we do not report our results on this task in our main paper. Instead, we include our preliminary evaluation procedure and results for this task in Appendix {\red [REF]}.
% }


% {\red ... Among other things, we should mention that any works that lead to progress on our tasks will necessarily increase the power of platforms to moderate content: this can be prosocial in the context of, e.g., preventing hate speech; but there are also concerns that this might be used for censorship (e.g., the following recent instance that Ashkan noticed: \url{https://www.nbcnews.com/tech/internet/viral-eyes-rafah-image-inspires-wave-ai-generated-instagram-posts-isra-rcna154555}) ...

% {\olv
% The limited shape perception abilities of these models could also be hypothetically exploited by malicious users to, e.g., disseminate hateful or sensitive material online by bypassing inappropriate content filters whose perceptual modules would not recognize the presence of inappropriate objects camouflaged through complex visual transformations.
% }
% }


==> results/DG_result.tex <==
\begin{table}
\centering
\small
\caption{\textbf{Domain Generalization}}
\label{tab:dg_res}
\resizebox{.95\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
 & \textbf{Cloud} & \textbf{Forest} & \textbf{Ocean} & \textbf{Origami} & \textbf{Sand Dune} \\
\midrule
\multicolumn{6}{c}{\textbf{Zeroshot \& Prompt Learning}} \\
\midrule
Zeroshot & 15.83 & 25.00 & 37.50 & 27.50 & 22.50 \\
DPLCLIP & 25.83 & 42.50 & 41.25 & 31.25 & 35.00 \\
\midrule
\multicolumn{6}{c}{\textbf{Linear Probing}} \\
\midrule
ERM & 31.25 & 57.50 & 48.75 & 45.00 & 57.50 \\
MixUp & 35.41 & 47.50 & 45.00 & 43.75 & 48.75 \\
GroupDRO & 33.13 & 51.25 & 48.75 & 42.50 & 48.75 \\
\midrule
\multicolumn{6}{c}{\textbf{Full Parameter Finetuning}} \\
\midrule
ERM & 90.83 & 83.75 & 87.50 & 87.50 & 82.50 \\
MixUp & 93.33 & 86.25 & 83.75 & 85.00 & 78.75 \\
GroupDRO & 93.33 & 81.25 & 85.00 & 78.75 & 76.25 \\
\bottomrule
\end{tabular}}
\end{table}
